Generic Library Interception for Improved Performance Measurement and Insight

As applications grow in capability, they also grow in complexity. This complexity in turn gets pushed into modules and libraries. In addition, hardware configurations become increasingly elaborate, too. These two trends make understanding, debugging and analyzing the performance of applications more and more difficult. To enable detailed insight into library usage of applications, we present an approach and implementation in Score-P that supports intuitive and robust creation of wrappers for arbitrary C/C++ libraries. Runtime analysis then uses these wrappers to keep track of how applications interact with libraries, how they interact with each other, and record the exact timing of their functions.

==> Makefile <==
PAPER_TEX = paper.tex
PAPER_PDF = paper.pdf
PAPER_AUX = paper.aux
PAPER_BIB = paper-references.bib

FIGURES = \
	figures/gromacs-1.png \
	figures/gromacs-2.png \
	figures/qt_libwrap_profile.png \
	figures/permon.png \
	figures/scorep_architecture.pdf \
	figures/software_stack.pdf \
	figures/workflow.pdf

LATEX_OUTPUT_FILTER = \
	grep -v ASDFASDFASDF | \
	grep -v PLACE_HOLDER_FOR_MORE_FILTERS

RED=`echo '\033[0;31m'`
YELLOW=`echo '\033[0;33m'`
BLUE=`echo '\033[0;34m'`
NOCOLOR=`echo '\033[m'`
BOLD=`echo '\033[1m'`
NORMAL=`echo '\033[0m'`

COLORIZE = \
	sed "s/Overfull/${RED}${BOLD}&${NORMAL}${NOCOLOR}/g" | \
	sed "s/Underfull/${YELLOW}${BOLD}&${NORMAL}${NOCOLOR}/g" | \
	sed "s/[0-9]*--[0-9]*/${BLUE}${BOLD}&${NORMAL}${NOCOLOR}/g" | \
	sed "s/LaTeX Warning/${YELLOW}${BOLD}&${NORMAL}${NOCOLOR}/g" | \
	sed "s/! LaTeX Error/${RED}${BOLD}&${NORMAL}${NOCOLOR}/g" | \
	sed "s/! Undefined control sequence/${RED}${BOLD}&${NORMAL}${NOCOLOR}/g" | \
	sed "s/l\.[0-9]*/${BLUE}${BOLD}&${NORMAL}${NOCOLOR}/g"

all: $(PAPER_PDF)

.IGNORE: $(PAPER_PDF)
$(PAPER_PDF): $(PAPER_TEX) $(FIGURES) $(PAPER_BIB) llncs.cls splncs03.bst

	@echo ">>> PRERUN PDFLATEX <<<"
	@echo ""
	pdflatex -shell-escape -interaction=nonstopmode --halt-on-error $(PAPER_TEX) 1> /dev/null 2> /dev/null
	@echo ""
	@echo ">>> BIBTEX <<<"
	@echo ""
	bibtex $(PAPER_AUX)
	@echo ""
	@echo ">>> PRERUN PDFLATEX <<<"
	@echo ""
	pdflatex -shell-escape -interaction=nonstopmode --halt-on-error $(PAPER_TEX) 1> /dev/null 2> /dev/null
	@echo ""
	@echo ">>> PDFLATEX <<<"
	@echo ""
	pdflatex -shell-escape -interaction=nonstopmode --halt-on-error $(PAPER_TEX) | $(LATEX_OUTPUT_FILTER) | $(COLORIZE)

.PHONY: clean
clean:
	rm -f *.aux *.dvi  *.idx *.ilg *.lof *.log *.lot *.out *.toc
	rm -f *.blg *.bbl *~ *.fdb_latexmk *.synctex.gz
	rm -f paper.pdf

